Kalman-Inspired Feature Propagation for Video Face Super-Resolution

Despite the promising progress of face image super-resolution, video face super-resolution remains relatively under-explored. Existing approaches either adapt general video super-resolution networks to face datasets or apply established face image super-resolution models independently on individual video frames. These paradigms encounter challenges either in reconstructing facial details or maintaining temporal consistency. To address these issues, we introduce a novel framework called Kalman-inspired Feature Propagation (KEEP), designed to maintain a stable face prior over time. The Kalman filtering principles offer our method a recurrent ability to use the information from previously restored frames to guide and regulate the restoration process of the current frame. Extensive experiments demonstrate the effectiveness of our method in capturing facial details consistently across video frames. Code and video demo are available at https://jnjaby.github.io/projects/KEEP.

==> figure/bar_var.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\linewidth]{figs/psnr_var.pdf}
    \vspace{-0.4cm}
    \includegraphics[width=.98\linewidth]{figs/ids_var.pdf}
    \vspace{-0.2cm}
    \caption{PNSR and IDS on different difficulty partitions.}
    \label{fig:bar_var}
    \vspace{-0.5cm}
\end{figure}

==> figure/histogram.tex <==
\begin{figure}[t]
    \centering
    \vspace{-0.3cm}
    \includegraphics[width=\linewidth]{figs/histogram.pdf}
    \caption{Histogram of $\mathcal{K}$ values. \cavan{in which equation? Can we give a more complete caption? And the font size is too small.}}
    \label{fig:histogram}
    \vspace{-0.5cm}
\end{figure}

==> figure/motivation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\linewidth]{figs/motivation.pdf}
    \vspace{-0.2cm}
    \caption{
    We show three frames with an interval of $5$. Single-image FSR model CodeFormer~\cite{zhou2022codeformer} hallucinates unnatural and inconsistent face details.
    Generic VSR model BasicVSR~\cite{chan2021basicvsr} fails to reconstruct facial components faithfully.
    Our method, in contrast, enables consistent restoration of low-quality face video while preserving temporal coherence across frames. \cavan{Convert this figure as our teaser figure. Show more frames. Also, encourage readers to watch the supplementary video to appreciate the superiority of our approach in terms of temporal consistency.}}
    \label{fig:motivation}
    \vspace{-0.5cm}
\end{figure}

==> figure/non_frontal.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\linewidth]{figs/non_frontal.pdf}
    \vspace{-0.3cm}
    \caption{\textbf{Comparisons on non-frontal faces.}
    While CodeFormer fails to restore eyes to these challenging cases, our method can still produce plausible facial elements.
    % \lichongyi{we may need to highlight that although our method is based on CodeFormer, it can handle the cases where CoderFormer does not work well. The reviewers may not get what information we would like to deliver.}
    }
    \label{fig:non_frontal}
    \vspace{-0.5cm}
\end{figure}
